X-lifecycle Learning for Cloud Incident Management using LLMs

Incident management for large cloud services is a complex and tedious process and requires significant amount of manual efforts from on-call engineers (OCEs). OCEs typically leverage data from different stages of the software development lifecycle [SDLC] (e.g., codes, configuration, monitor data, service properties, service dependencies, trouble-shooting documents, etc.) to generate insights for detection, root causing and mitigating of incidents. Recent advancements in large language models [LLMs] (e.g., ChatGPT, GPT-4, Gemini) created opportunities to automatically generate contextual recommendations to the OCEs assisting them to quickly identify and mitigate critical issues. However, existing research typically takes a silo-ed view for solving a certain task in incident management by leveraging data from a single stage of SDLC. In this paper, we demonstrate that augmenting additional contextual data from different stages of SDLC improves the performance of two critically important and practically challenging tasks: (1) automatically generating root cause recommendations for dependency failure related incidents, and (2) identifying ontology of service monitors used for automatically detecting incidents. By leveraging 353 incident and 260 monitor dataset from Microsoft, we demonstrate that augmenting contextual information from different stages of the SDLC improves the performance over State-of-The-Art methods.

==> Figures/inc_only.tex <==
% Prompt - without dependency details, with historical incidents
\begin{figure}[t]
\ffbox{
\textbf{-- Task Description:} \\

- You are dealing with root cause analysis for Azure cloud incident. You are an \textbf{**on-call engineer**} that is responsible for investigating the root cause.

- You will be provided with the title and summary of the incident along with the service name and functionality that is affected by the incident.  

- In the context of software engineering and system architecture, an upstream service dependency denotes a relationship between two services, where one service (the dependent service) relies on another service (the dependency) to fulfill its operational requirements. This dependency typically involves the exchange of data, execution of functions, or access to resources necessary for the dependent service to perform its intended tasks. This relationship is termed "upstream" to signify the flow of dependencies from the dependent service to its sources, akin to the flow of a river from its upstream source. \\

\textbf{-- Historical Incident Examples:}

- Below are some historical incidents with their root causes. If you find the description and title to be \textbf{**similar or relevant**} to the current incident, you can also use the examples to determine the root cause of the current incident. \\

- Historical Incident Summary 1: {Retrieved summary}

- Historical Incident Title 1: {Retrieved title}

- Historical Incident Root Cause 1: {Retrieved Root cause} \\
... ... \\
- Historical Incident Summary 5: {Retrieved summary }

- Historical Incident Title 5: {Retrieved title}

- Historical Incident Root Cause 5: {Retrieved Root cause}\\


\textbf{-- Answering Format:} Your output response should strictly be a **Json** file with the following two objectives: \\

\textbf{Objective1:} Infer and explain in detail, the Root cause that could have caused the incident 

\textbf{Objective2:} Binary classification as follows: If and only if you identify the root cause as an upstream service dependency, return "Yes". Else, if the incident is \textbf{**not**} caused due to the failure of an upstream service, return "No"  
\\

\textbf{-- Incident Details:}  \\
- Service: {Service Name} 

- Functionality: {Functionality of the Service} 

- Incident Summary: {The summary of the incident} 

- Incident Title: {Title of the incident} 
\\
}
\caption{Prompt with in-context historical incident examples along with the Incident metadata}
\label{fig:inc_only}
\end{figure}

==> Figures/incident_only.tex <==
\begin{figure}[t]
% vanilla prompt - without dependency details/historical incidents
\ffbox{
\textbf{-- Task Description:} \\

- You are dealing with root cause analysis for Azure cloud incident. You are an **on-call engineer** that is responsible for investigating the root cause. 

- You will be provided with the title and summary of the incident along with the service name and functionality that is affected by the incident.  

- In the context of software engineering and system architecture, an upstream service dependency denotes a relationship between two services, where one service (the dependent service) relies on another service (the dependency) to fulfill its operational requirements. This dependency typically involves the exchange of data, execution of functions, or access to resources necessary for the dependent service to perform its intended tasks. This relationship is termed "upstream" to signify the flow of dependencies from the dependent service to its sources, akin to the flow of a river from its upstream source. 
 \\
 
\textbf{-- Answering Format:} Your output response should strictly be a **Json** file with the following two objectives: 
\\
\textbf{Objective1:} Infer and explain in detail, the Root cause that could have caused the incident 

\textbf{Objective2:} Binary classification as follows: If and only if you identify the root cause as an upstream service dependency, return "Yes". Else, if the incident is **not** caused due to the failure of an upstream service, return "No"  
\\

\textbf{-- Incident Details:}  \\
- Service: {Service Name} 

- Functionality: {Functionality of the Service} 

- Incident Summary: {The summary of the incident} 

- Incident Title: {Title of the incident}
}
\caption{Baseline prompt with Incident metadata}
\label{fig:incident_only}
\end{figure}

==> Figures/incident_w_dep.tex <==
% Prompt - with dependency details, without historical incidents
\begin{figure}[t]
\ffbox{
\textbf{-- Task Description:} \\

- You are dealing with root cause analysis for Azure cloud incident. You are an \textbf{**on-call engineer**} that is responsible for investigating the root cause.

- You will be provided with the title and summary of the incident along with the service name and functionality that is affected by the incident.  

- You will also be provided with a list of \textbf{** Upstream service dependencies**} and their \textbf{**Descriptions**}

- In the context of software engineering and system architecture, an upstream service dependency denotes a relationship between two services, where one service (the dependent service) relies on another service (the dependency) to fulfill its operational requirements. This dependency typically involves the exchange of data, execution of functions, or access to resources necessary for the dependent service to perform its intended tasks. This relationship is termed "upstream" to signify the flow of dependencies from the dependent service to its sources, akin to the flow of a river from its upstream source. 

- The Upstream service dependencies have been provided so that you can better identify the root cause of the incident  \\ 

\textbf{-- Answering Format:} Your output response should strictly be a **Json** file with the following two objectives: \\

\textbf{Objective1:} Infer and explain in detail, the Root cause that could have caused the incident 

\textbf{Objective2:} Binary classification as follows: If and only if you identify the root cause as an upstream service dependency, return "Yes". Else, if the incident is \textbf{**not**} caused due to the failure of an upstream service, return "No"  
\\

\textbf{-- Incident Details:}  \\
- Service: {Service Name} 

- Functionality: {Functionality of the Service} 

- Incident Summary: {The summary of the incident} 

- Incident Title: {Title of the incident} 
\\

\textbf{-- Upstream Service Dependencies:}

1. Upstream Service Name – {Description of the Upstream Service} 
... ....  \\
 n. Upstream Service Name – {Description of the Upstream Service}
}
\caption{Prompt with additional Upstream service details}
\label{fig:incident_w_dep}
\end{figure}

==> Figures/slo_class.tex <==
\begin{figure}[t]
\ffbox{
\textbf{-- Task Description:} \\
- You are an intelligent software engineer who answers questions from a user based on the monitor metadata provided. A Service Level Objective (SLO) is a target or goal for the level of service that a system or service should provide. It is a specific, measurable, and time-bound objective that helps define the quality of service that a customer or user can expect. Go through service description and monitor metadata \{'Monitor Name', 'Account Name', 'namespace', 'Metric name', 'Sampling Type', 'Alert Title', 'Service Name'\}, preprocess the text such as camel casing, snake case splitting, etc. to decode any service specific tokens and predict the service level objectives being tracked by the monitor. Use service description only if you need additional context. And answer the following questions about the monitor sequentially. \\

1. Q1. What do you think is the service level objective tracked by this monitor? Provide justifications for your output? \\
2. Q2: Categorize the service level objective being tracked by the monitor to a generic class: 
\begin{enumerate}
    \item Availability
    \item Latency
    \item Capacity
    \item Throughput
    \item SuccessRate
    \item Interruption Rate
    \item Freshness 
    \item Reliability
    \item Others
\end{enumerate}

\medskip
\textbf{-- Additional Guidance :} \\

- Focus on extracting relevant information from the descriptions. 

- Pay attention to specific features or characteristics indicative of the resource class. 

- Consider negations or exceptions in descriptions. 

- Highlight the importance of understanding relationships between different elements. 
}
\caption{Prompt for generating SLO class labels}
\label{fig:enter-label}
\end{figure}

==> Tables/f1_acc_rca.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\centering
% \tabcolsep=0.08cm
\begin{tabular}{ll cccc}
\toprule
& & NoDEP & DEP & InC NoDEP & InC DEP \\ \midrule
\multirow{2}{*}{F1}       & Ovr    & 47.330 & \textbf{50.935} & 35.561 & 39.763 \\
                          & Dep & 39.316 & \textbf{57.576} & 15.686 & 56.489 \\ \bottomrule
% \multirow{2}{*}{Accuracy} & Ovr    & \emph{51.558} & \textbf{51.558} & 45.326 & 36.261 \\
%                           & Dep & 24.468 & \textbf{40.426} & 8.511  & 39.362 \\ \bottomrule
\end{tabular}
\vspace{2mm}
\caption{In this table, we assess the model's ability to predict whether an incident is due a service dependency failure. We use the F1 and Accuracy metrics. \todo{Check the next line For the same we used F1 and Accuracy metrics where we can see adding In-Context examples does not help in classification. And the reason might be the noise from these examples that confusing the model.}
%can we modify the title? And do we need to highlight the fact part about the contextual examples in the tile itself?
\emph{Ovr}: denotes Overall i.e., for all samples, while \emph{Dep}: All those incidents caused from service dependency.}
\label{tab:my-table}
\end{table}

==> Tables/resource.tex <==
\begin{table}[t]
\centering
\caption{Quantitative metrics evaluated on Resource Class recommendations.}
% \tabcolsep=0.08cm
% \small
\begin{tabular}{l cccc} 
\toprule
Resource Class    & Precision & Recall & f1-score & Accuracy \\ \midrule
Service level     & 0.47      & 0.22   & 0.30     & 0.26     \\
API               & 0.43      & 0.83   & 0.56     & 0.83     \\
CPU               & 0.62      & 1.00   & 0.76     & 1.00     \\
Container         & 1.00      & 0.57   & 0.73     & 0.59     \\
Dependency        & 0.76      & 0.50   & 0.60     & 0.54     \\
Compute cluster   & 0.71      & 0.50   & 0.59     & 0.52     \\
Storage           & 0.59      & 0.76   & 0.67     & 0.83     \\
Ram-memory        & 1.00      & 1.00   & 1.00     & 1.00     \\
Certificate       & 0.96      & 1.00   & 0.98     & 1.00        \\
Cache-memory      & 0.90      & 0.95   & 0.93     & 1.00     \\
IO                & 0.70      & 0.89   & 0.78     & 0.89     \\
Paging Memory     & 0.93      & 0.88   & 0.90     & 0.93     \\
None-of-the-above & 0.33      & 0.05   & 0.09     & 0.06     \\ \bottomrule
\end{tabular}
\end{table}


==> Tables/resource_baseline.tex <==
\begin{table}[t]
\centering
\caption{Quantitative metrics evaluated on Resource Class recommendations (baseline).}
% \tabcolsep=0.07cm
% \small
\begin{tabular}{l cccc} 
\toprule
Resource Class    & Precision & Recall & f1-score & Accuracy \\ \midrule
Service level     & 0.48      & 0.33   & 0.39     & 0.39    \\
API               & 0.44      & 0.72   & 0.55     & 0.78     \\
CPU               & 0.63      & 0.90   & 0.75     & 1.00     \\
Container         & 1.00      & 0.63   & 0.77     & 0.67     \\
Dependency        & 0.64      & 0.47   & 0.55     & 0.50     \\
Compute cluster   & 0.69      & 0.38   & 0.49     & 0.47     \\
Storage           & 0.72      & 0.92   & 0.81     & 0.92     \\
Ram-memory        & 1.00      & 0.83   & 0.91     & 0.95     \\
Certificate       & 1.00      & 1.00   & 1.00     & 1.00        \\
Cache-memory      & 0.81      & 0.85   & 0.83     & 1.00     \\
IO                & 0.76      & 0.89   & 0.82     & 0.94     \\
Paging Memory     & 0.93      & 0.88   & 0.90     & 0.93     \\
None-of-the-above & 0.00      & 0.00   & 0.00     & 0.00     \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/slo.tex <==
\begin{table}[t]
\caption{Quantitative metrics evaluated on SLO recommendations.}
% \tabcolsep=0.08cm
% \small
\begin{tabular}{l cccc } 
\toprule
SLO Class         & precision & recall & f1-score & accuracy \\ \midrule
Availability            & 0.48      & 1.00   & 0.65     &          \\
Capacity                & 0.90      & 0.64   & 0.75     &          \\
Freshness               & 1.00      & 0.75   & 0.86     &          \\
Interruption Rate       & 1.00      & 0.31   & 0.47     &          \\
Latency                 & 0.88      & 1.00   & 0.94     &          \\
Others                  & 0.00      & 0.00   & 0.00     &          \\
Success Rate - QoS      & 0.96      & 0.92   & 0.94     &          \\
Success Rate            & 0.92      & 0.55   & 0.69     &          \\
Throughput              & 0.87      & 0.93   & 0.90     &          \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/slo_baseline.tex <==
% \begin{table}[t]
% \caption{Quantitative metrics evaluated on SLO recommendations.}
% \centering
% % \tabcolsep=0.03cm
% % \small
% \begin{tabular}{l cccc}
% \toprule
% Resource Class    & Precision & Recall & f1-score & Accuracy \\ \midrule
% Service level     & 0.45      & 0.25   & 0.32     & 0.28     \\
% API               & 0.36      & 0.72   & 0.48     & 0.78     \\
% CPU               & 0.66      & 1.00   & 0.79     & 1.00     \\
% Container         & 1.00      & 0.49   & 0.65     & 0.53     \\
% Dependency        & 0.43      & 0.50   & 0.46     & 0.56     \\
% Compute cluster   & 0.80      & 0.50   & 0.62     & 0.55     \\
% Storage           & 0.63      & 0.88   & 0.73     & 0.96     \\
% Ram-memory        & 1.00      & 0.83   & 0.91     & 1.00     \\
% Certificate       & 0         & 0      & 0        & 0        \\
% Cache-memory      & 0.36      & 0.72   & 0.48     & 0.78     \\
% None-of-the-above & 0.36      & 0.72   & 0.48     & 0.78     \\ \bottomrule
% \end{tabular}
% % \label{tab:desc_results_resource}
% \end{table}
\begin{table}[t]
\centering
\caption{Quantitative metrics evaluated on SLO recommendations (baseline).}
\begin{tabular}{l cccc}
\toprule
SLO Class         & precision & recall & f1-score & accuracy \\
\midrule
Availability      & 0.45      & 0.85   & 0.59     &          \\
Capacity          & 0.89      & 0.57   & 0.70     &          \\
Freshness         & 1.00      & 0.67   & 0.80     &          \\
Interruption Rate & 1.00      & 0.23   & 0.38     &          \\
Latency           & 0.82      & 1.00   & 0.90     &          \\
Others            & 0.00      & 0.00   & 0.00     &          \\
Success Rate - QoS       & 0.87      & 0.94   & 0.90     &    \\
Success Rate      & 0.85      & 0.55   & 0.67     &          \\
Throughput        & 0.87      & 0.93   & 0.90     &          \\
\bottomrule
\end{tabular}
\end{table}
